Reconstruction Attacks on Aggressive Relaxations of Differential Privacy

Differential privacy is a widely accepted formal privacy definition that allows aggregate information about a dataset to be released while controlling privacy leakage for individuals whose records appear in the data. Due to the unavoidable tension between privacy and utility, there have been many works trying to relax the requirements of differential privacy to achieve greater utility. One class of relaxation, which is starting to gain support outside the privacy community is embodied by the definitions of individual differential privacy (IDP) and bootstrap differential privacy (BDP). The original version of differential privacy defines a set of neighboring database pairs and achieves its privacy guarantees by requiring that each pair of neighbors should be nearly indistinguishable to an attacker. The privacy definitions we study, however, aggressively reduce the set of neighboring pairs that are protected. Both IDP and BDP define a measure of "privacy loss" that satisfies formal privacy properties such as postprocessing invariance and composition, and achieve dramatically better utility than the traditional variants of differential privacy. However, there is a significant downside - we show that they allow a significant portion of the dataset to be reconstructed using algorithms that have arbitrarily low privacy loss under their privacy accounting rules. We demonstrate these attacks using the preferred mechanisms of these privacy definitions. In particular, we design a set of queries that, when protected by these mechanisms with high noise settings (i.e., with claims of very low privacy loss), yield more precise information about the dataset than if they were not protected at all.

==> GroupKReconstruction.tex <==
\begin{comment}

\begin{definition}[K-Local Sensitivity]
The local sensitivity of a function $f$ with respect to a dataset $D$ (denoted as $\Lambda_K(f,D)$ is defined as the largest change in $f$ that can be achieved by modifying K records in $D$. Let $\mathcal{N}$ be the set of neighbors of $D$ obtained by modifying up to K records:

\begin{equation}
    \Lambda_K(f,D) = \max_{D^\prime\in \mathcal{N}} ||f(D) - f(D^\prime)||
\label{eqn:GroupSens}
\end{equation}
\end{definition}

% not directly quoted, more of an adaptation. not 100% sure if this is what they were intending? If incorrect, we might need to adjust this definition and include a lemma that shows that the privacy guarantee for individuals should be higher for higher K, and that we can break it at K anyway
\begin{definition}[Group K Differential Privacy \cite{idp}]
Given a data set $D$, a response mechanism $\kappa$ satisfies Group-K differential privacy if for any dataset $D'$ at distance of at most $K$ from $D$ and $S \subset Range(\kappa)$:

\begin{equation}
    exp(-\epsilon)Pr(\kappa(D') \in S) \le Pr(\kappa(D) \in S) \le exp(\epsilon)Pr(\kappa(D') \in S)
    \label{eqn:GroupPriv}
\end{equation}
\end{definition}

One proposed method of ensuring Group K differential privacy proposes to add noise to the answer of a function, where the amount of noise depends on the K-local sensitivity.

\begin{definition}[kDP Laplace Mechanism]
Let $f$ be a function whose output is a vector. Let $\epsilon > 0$ be a privacy parameter and let $M$ be a mechanism that, on input $D$, adds independent Laplace noise with scale $\Lambda_K(f, D)/\epsilon$ to each component of $f$ (i.e. $M(D) = f(D) + \text{Laplace}(\Lambda_K(f, D)/\epsilon)$. This $M$ is called a $\epsilon-kDP$ Laplace Mechanism
\end{definition}

\end{comment}


In this section, we will now show how the Count query can be adapted to obtain private information from a privacy mechanism satisfying K $\epsilon$-IDP. 
Algorithm \ref{algo:KSensitivity} represents the mechanism through which a data custodian with complete visibility to the actual database will answer queries on Equation \ref{eqn:fnv} through the K $\epsilon$-IDP mechanism. The algorithm takes the original database D, inclusive lower count range U, exclusive upper count range V, group size K representing the number of records that can change in the neighbors of D, b from Equation \ref{eqn:fnv}, the privacy parameter $\epsilon$ and column number indicator i as input parameters. It is important to note that the algorithm asserts that size of the database at-least needs to be greater or equal to twice the chosen value of K. Taking into account that K elements  can change in the local neighbors, the count of range, $\mathcal{R}$= $\left[u, v\right)$ of items in the database column, D[i], can vary from maximum(count($\mathcal{R}$)$_{D[i]}$-K, 0) to minimum(count($\mathcal{R}$)$_{D[i]}$+K, size(D[i])) in the K-local sensitivity bounded neighboring databases. The K-local sensitivity is 0 when b $<$ maximum(count($\mathcal{R}$)$_{D[i]}$+K, 0) or when b$\geq$minimum(count($\mathcal{R}$)$_{D[i]}$+K, size(D[i])), other values of b generates a K-local sensitivity equal to 1. 

% \begin{example}
% To illustrate this sensitivity calculation mechanism, assume a database, D = [5,8,9,16,17,20]. Let's look at the case of K = 2 and when u and v are initially 1 and 10 respectively, meaning $\mathcal{R}$ = $\left[1, 10\right)$ returns the count of the first three elements in the database. Now, the true count($\mathcal{R}$)$_D$ = 3. In the K-local neighboring databases of D, count can change from maximum(3-2, 0)=1 (consider D' = [12,12,9,16,17,20]) to minimum(3+2, 6)=5 (consider D'' = [5,8,9,8,8,20]). Considering b$<$1, let's work with the edge case of b=0. Count($\mathcal{R}$)$_D$=3 as well as count($\mathcal{R}$)$_{D'}$=1 and count($\mathcal{R}$)$_{D''}$=5 are greater than b, when b=0. So the K-local sensitivity for b$<$1 is 0. Next, let's look at the case when b$\geq$5, once again let's take the edge case b=5, none of count($\mathcal{R}$)$_{D}$=3, count($\mathcal{R}$)$_{D'}$=1 and count($\mathcal{R}$)$_{D''}$=5 are greater than b. The K-local sensitivity once again is 0. Next, let's examine the case when 1$\geq$b$<$5, let's take b=4. Now, count($\mathcal{R}$)$_{D}$=3 is not greater than 4, but count($\mathcal{R}$)$_{D''}$=5 is greater than 4. Similarly, when b=1, count($\mathcal{R}$)$_{D}$=3 is greater than 1, but count($\mathcal{R}$)$_{D'}$=1 is not greater than 1. For 1$\geq$b$<$5, the K-local sensitivity is 1 (difference between of outputs of Equation \ref{eqn:fnv} on D and it's K-local neighbors). 
% \end{example}


\begin{algorithm}
\caption{K $\epsilon$-IDP Query Answering Mechanism For Equation Equation \ref{eqn:fnv}}
\begin{algorithmic}[1]

\Function{Count}{D,U,V,K,b,$\epsilon$,i}
\State assert D[i].size() $\geq$ 2K
     \State DSubset := [x for x in D[i] where x $\geq$ U and x $<$ V]
     \State LowerBound := Max(DSubset.size() - K, 0)
     \State UpperBound := Min(DSubset.size() + K -1, D[i].size())

     \If{b $<$ LowerBound}
         \State \Return 1
     \ElsIf{b $>$ UpperBound}
         \State \Return 0
     \Else
         \State \Return ((DSubset.size()$>$b) + Laplace(1/$\epsilon$))
     \EndIf 
    

 \EndFunction

 \end{algorithmic}\label{algo:KSensitivity}
 \end{algorithm}

\begin{lem}
\label{lem:countKObservation}
The observed outputs of querying $f_{b,u,v}$ on a database column $D$[i] hold: if the observed output of $f_{b,u,v}$ is 0, then there are are fewer than b elements in the range $\mathcal{R} = \left[u, v\right)$ in the database column. If the observed output of $f_{b,u,v}$ is 1, then there are greater than b elements in D[i]. If the observed value is decimal, then $count(\mathcal{R}_{D[i]}) - K \le b < count(\mathcal{R}_{D[i]}) + K$.
\end{lem}

\begin{proof}
We can measure the K-local sensitivity of our output by whether we observe a binary or non-binary number. If we observe a binary number, then we know the K-local sensitivity must be 0 because any noise from a continuous Laplacian distribution would almost certainly create decimal values. Similarly, we can see that if we observe a decimal value, then the K-local sensitivity must not be 0, and therefore must be 1 because it is impossible for $f_{b,u,v}$ to have a sensitivity that is not 1 or 0.

Suppose we observe a decimal value. Then, the K-local sensitivity must be equal to 1. By lemma \ref{lem:countKSensitivity}, we know that the K-local sensitivity of $f_{b,u,v}(D[i])$ is 1 when $count(\mathcal{R}_{D[i]}) - K \le b < count(\mathcal{R}_{D[i]}) + K$, and 0 otherwise. Thus, for this query, it must be true that $count(\mathcal{R}_{D[i]})-K \le b < count(\mathcal{R}_{D[i]}) + K$. Suppose we observe a binary value. Then, the K-local sensitivity must be equal to 0. By lemma \ref{lem:countKSensitivity}, we know that the K-local sensitivity of $f_{b,u,v}(D[i])$ is 0 when $b < count(\mathcal{R}_{D[i]})-K$ or $b \ge count(\mathcal{R}_{D[i]})+K$, and 1 otherwise. Thus, if we observe a binary value, b must satisfy one of the above conditions. Since the K-local sensitivity of the function is 0, we will observe its true value.

If we observe 1, then by the definition of $f_{b,u,v}$, we know that $count(\mathcal{R}_{D[i]}) > b$. Thus, $count(\mathcal{R}_{D[i]}) + K > b$, and it cannot be the case that $b \ge count(\mathcal{R}_{D[i]})$. Therefore, it must be true that $b < count(\mathcal{R}_{D[i]}) - K$. If we observe 0, then by the definition of $f_{b,u,v}$, we know that $count(\mathcal{R}_{D[i]}) \le b$. Thus, $count(\mathcal{R}_{D[i]}) - K < b$, and it cannot be the case that $b < count(\mathcal{R}_{D[i]}) - K$. Therefore, it must be true that $b \ge count(\mathcal{R}_{D[i]}) + K$
\end{proof}

The above lemmas demonstrate that the binary count query has a similar behavior when called on a database protected by the K $\epsilon$-IDP  mechanism versus when called on the $\epsilon$-IDP mechanism. The only difference between the two is the size of the range of b for which Equation \ref{eqn:fnv} gives a decimal value, which is 2 for IDP and up to 2K for the group variant. Because the range of values for b could be upper bounded by either 0 or the size of the database, we must find an upper boundary to deduce the count of an element when the true count is within K of 0, and we must find a lower boundary when the true count is within K of Size(D). Upon discovering an upper or lower threshold between decimal and binary values for b-1 and b, it can be deduced that the true count of values in the given range is b+K for a lower threshold and b-K for an upper threshold. We can use b to perform a binary search on a database to find such thresholds and deduce the true count according to algorithm \ref{alg:groupKCount}.

The above lemma enables us to use b to perform a binary search on a database column and find a threshold between non-binary and binary values using much the same process as used in the IDP mechanism. Algorithm \ref{alg:groupKCount} represents the process of utilizing the query answering mechanism from Equation \ref{eqn:fnv} to accurately find the frequency occurrence of elements in range $\mathcal{R}$=[u,v) in database column, D[i], given size(D[i]) $\geq$2K. The algorithm uses a binary search to find the lowest b where Equation \ref{eqn:fnv} produces a decimal value and also the lowest b that generates a value of 0. We call these two boundary values of b as the left and right boundaries respectively. A decimal value output from Equation \ref{eqn:fnv} for b and a binary value for b$-$1 gives the indication that b is the left boundary and b+K is a possibility for the actual count of elements in range [u,v) in D. A decimal value output from Equation \ref{eqn:fnv} for b-1 and a binary value for b gives the indication that b is the right boundary and b-K is another possibility for the actual count of elements in range [u,v) in D. Both binary value outputs for b and (b$-$1) means that either b-1$\geq$minimum(count($\mathcal{R}$)$_{D}$+K, size(D)) or b$<$maximum(count($\mathcal{R}$)$_{D}$-K, 0). Both non-binary value outputs for b and (b$-$1) means that b-1$\geq$maximum(count($\mathcal{R}$)$_{D}$-K, 0) and b $<$minimum(count($\mathcal{R}$)$_{D}$+K, size(D)). If the left boundary is 0 or if the right boundary is size(D), then there is a possibility that (left boundary + K) or (right boundary - K) is not the true count of range $\mathcal{R}$, since the K is limited by the size of the database. We avoid such cases and take (left boundary + K) as the true count when left boundary > 0 and take (right boundary - K) as the true count when right boundary < size(D). In the event that the left boundary is 0 and the right boundary is size(D), then both (left boundary + K) and (right boundary - K) will produce the true count since the true count resides right in the middle. 

\begin{algorithm}
\caption{K-Local Sensitivity Query Function - Get count of elements in Range}
\begin{algorithmic}[1]
\Function{GetRangeCount}{D,U,V,K,$\epsilon$,DSize,i}

    \State L := Find Lowest b with Binary Search: Algo 6 $\neq\{0,1\}$
    \State R := Find Lowest $b$ with Binary Search: Algo 6 $\xrightarrow{}$ 0
    
    \If{(L $>$ 0)}
        \State \Return L + K
    \ElsIf{(R $<$ DSize)}
        \State \Return R - K
    \Else
        \State \Return L + K
    \EndIf

\EndFunction
\end{algorithmic}\label{alg:groupKCount}
\end{algorithm}

We note that this process might not necessarily hold if the database has more than $2K$ elements. Since the number of elements in $\mathcal{R}$ could vary up to K in either direction, bounded by the size of the database, it would be possible that there could be multiple ranges for which $count(\mathcal{R}) - K$ and $count(\mathcal{R}) + K$ are outside the range of the database. Then, the K-local sensitivity of $f_{b,u,v}$ would be 1 for all $b \in \left[0, size(D) \right]$. Thus, there would be no transition between a binary and non-binary value inside the boundary of the database, so we could not reconstruct the true count of elements inside $\mathcal{R}$. Since there could be multiple ranges of values with this property, it is also not necessarily possible that we would be able to calculate the count in the range by subtracting the sum of the counts of remaining values from size(D).

% \begin{example}
% To illustrate how the count of elements in range D can be deduced through algorithm 9, let us consider a group size K=2 and a Database, D = [5,8,9,16,17,20]. Let's look at the case when u and v are 1 and 10 respectively, meaning $\mathcal{R}$ = [1, 10) returns the count of the first three elements in the database. Now, the true count($\mathcal{R}$)$_{D}$ = 3. In the K-local neighboring databases of D, count can change from maximum(3-2, 0)=1 (consider D' = [12,12,9,16,17,20]) to minimum(3+2, 6)=5 (consider D'' = [5,8,9,8,8,20]). When b$<$1, consider the case when b$=$0 and b$-$1$=-$1, Equation \ref{eqn:fnv} would output 1 for both of these cases since the K-local sensitivity is 0 and count($\mathcal{R}$)$_{D}$ of 3 $>$ b and b$-$1. When b$-$1$\geq$5, consider b=6 and b$-$1=5, both these cases would produce a output of 0 when Equation \ref{eqn:fnv} is applied since K-local sensitivity is still 0 and count($\mathcal{R}$)$_{D}$ of 3 $<$ b and b$-$1. When b$<$5 and b-1$\geq$1, consider the case of b=4 and b$-$1=3, both these cases would produce a non-binary output when Equation \ref{eqn:fnv} is applied since K-local sensitivity is 1. One interesting case is seen when b=1 and b$-$1=0, b=1 would produce a non-binary output (K-local sensitivity = 1) and b$-$1=0 would output 1(K-local sensitivity = 0) with Equation \ref{eqn:fnv}. The left boundary is found at b=1 as a result. The other interesting case is seen when b=5 and b$-$1=4, b-1 would produce a non-binary output (K-local sensitivity = 1) and b would output 0 (K-local sensitivity = 0) with Equation \ref{eqn:fnv}. This change from non-binary output to binary output tells us that b=5 is the right boundary. Now, both left boundary + K (1+2=3) and right boundary - K (5-2=3) produces the true count of count($\mathcal{R}$)$_{D}$. 
% \end{example}

% \begin{lem}
% \label{lem:countKReconstruction}
% Given a function $f_{b,u,v}$ as defined above, the number of elements in a given range in the database can be reconstructed by noticing the changes of the function output from a binary value to a non-binary value for different inputs of b when querying on the $\epsilon-kDP$ when the database has at least $2K$ elements.
% \end{lem}

% \begin{proof}
% Let $a_1 \le a_2 \le \cdots a_k \le a_{k+1} \le \cdots \le a_{k+m-1} \le \cdots \le a_n$ be the elements of D in non-decreasing order, where $n > 2K$. We see that $D$ has n total elements and m elements in the range $\mathcal{R} = \left[u, v\right)$, where $a_k$ is the first such element.

% We could view the case of individual differential privacy as being equivalent to group K differential privacy with K=1. Since the count function behaves similarly on kDP as iDP with a different range, the relationship between the decimal-binary boundary and the true count of elements in the range follow from lemma \ref{lem:countReconstruction}.

% Upon finding a lower boundary where querying the count function with b gives a decimal and querying on b-1 gives a binary number, and $b \ne 0$, we deduce that $m = b + k$. Upon finding an upper boundary where querying the count function on b gives a binary value and querying on b-1 gives a decimal value and $b \ne n$, we deduce that $m = b - k$.

% Now, for $b < m - K$, lemma \ref{lem:countKSensitivity} states that the K-local sensitivity is equal to 0. This means that Laplace noise added by the $\epsilon-idp$ mechanism will have variance equal to 0 (i.e. no noise will be added at all). Thus, in this case, querying $f_{b,u,v}$ will produce an output of 1. The identification of a binary result here is significant. Similarly, for $b \ge m + K$, lemma \ref{lem:countKSensitivity} states that the K-local sensitivity is equal to 0, which means querying $f_{b,u,v}$ will yield a binary result. However, in this case, the function $f_{b,u,v}$ outputs 0, instead of 1.

% Now, we consider the case of $m-K \le b < m+K$, where lemma \ref{lem:countKSensitivity} states that the function $f_{b,u,v}$ will have a K-local sensitivity of 1. In this case, noise will be drawn from a Laplace distribution with non-zero variance and added to the output of the function. Because Laplace noise is a continuous function, the output of $f_{b,u,v}$ in this case will almost always be equal to a non binary number.

% It follows from lemma \ref{lem:countKSensitivity} that $f_{b,u,v}$ generates a binary value for $b < m - K$ and $b \ge m + K$, and a non-binary value when $m - K \le v < m + K$. We start by querying the function with $b = 0$. If $m \ge K+1$, then our first query will yield a binary value. Then, we could repeatedly query while shifting b upwards in increments of 1 until the output changes from a binary to a non-binary value. The first decimal value will be seen when $b = m - K$, since we control $b$ to integer values and $m$ can only be an integer value. Thus, when the query output of $f_{b,u,v}$ changes from a binary value 1 to a non-binary value, we know that the true value of $m$ must be equal to $b + K$. 

% For $m \in \left[0, K\right]$, our first query for $b = 0$ will start with a decimal value. When our first query yields a non-binary value, we can instead watch for when the function switches from outputting a decimal value to outputting a binary value, still increasing b in increments of 1. Then, because lemma \ref{lem:countKSensitivity} tells us that the sensitivity for $f_{b,u,v}$ is equal to 0 when $m+K \le b$, the function will switch from outputting a decimal to binary value when $b = m+K$. Thus, we would be able to deduce that the true value of $m$ is equal to $b-K$.

% By lemma \ref{lem:countKObservation}, we could clearly optimize searching for these boundaries by applying binary search.
% \end{proof}

This technique can be used to reconstruct the entire database by querying with different upper bound values V to reveal records from the database. Algorithm \ref{alg:groupKReconstruction} demonstrates the process of reconstructing the entire database by calling the function from Algorithm \ref{alg:groupKCount} repeatedly. The algorithm starts with setting the upper-bound V and the lower-bound U to extremely large values such that the entire database is contained within U and V. For symbolic purposes, the large values are denoted as infinity and negative infinity in the algorithm itself. Algorithm \ref{alg:groupKCount} is called with the initial big U and V values to get the count of the entire database, which is stored in X and DSize. Next, a binary search is performed over possible values of V to find the largest V that produces a count value different from X. This new count value is denoted as Y. The largest V which generates Y is the largest element in the database and that V repeats X-Y times in the database. The algorithm then inserts V into the reconstructed database X-Y times and sets X to the found Y. The process is repeated until there are no more elements in the original database to be revealed.

\begin{algorithm}
\caption{Reconstruct Database Column Under Group K-IDP Setting}
\begin{algorithmic}[1]

\Function{Reconstruction}{D,$\epsilon$,K,i}
    
    \State V,U := $\infty$,$-\infty$
    \State ReconstructedColumn := [ ]   
    \State DSize := GetRangeCount(D,U,V,K,$\epsilon$,-1,i)  
    \State X := DSize

    \While{(X != 0)}  
    %\State Find Largest V with Binary Search when Alg 9 $\xrightarrow{}$Y $\neq$X
    \State Find Largest $N < V$ with Binary Search such that 
    \State GetRangeCount(D,U,N,K,$\epsilon$,DSize,i) returns Y $\neq X$

    \State Add V to ReconstructedColumn X-Y times
    \State X := Y

  
    \EndWhile \label{loop1}
    \State \Return ReconstructedColumn

\EndFunction

\end{algorithmic}\label{alg:groupKReconstruction}
\end{algorithm}


\subsection{Dataset reconstruction}\label{subsec:idpfull}


% \begin{example}
% To illustrate how the reconstruction will function, let's consider a Database, D = [8,8,15] and assume K=1. Initially calling algorithm 9 by setting u and v to be very large, let's call this range $\mathcal{R}$ = [$-\infty$,$\infty$), will return the count of the entire database, D. In our example, count($\mathcal{R}$)$_{D}$ = 3. This size of the the database will be set as the first current reference count.  Now, in algorithm 9, a binary search will be  performed over possible values of v such that for range $\mathcal{R}$ = [$-\infty$,v), count($\mathcal{R}$)$_{D}$ will generate a value of X which is not equal to the current reference count = 3 and range $\mathcal{R}$ = [$-\infty$,v + smallest increment) (smallest increment is 1 for data-sets that only contains integer value elements) generates count($\mathcal{R}$)$_{D}$ = current reference count. In database, D, for $\mathcal{R}$ = [$-\infty$,15), count($\mathcal{R}$)$_{D}$ generates a value of 2 which is not equal to 3 and for  $\mathcal{R}$ = [$-\infty$,15+1), count($\mathcal{R}$)$_{D}$ generates an output equal to 3. This binary search results tell us that V=15 is an element in the database and it repeats in the database 3-2=1 times. Next, the value  generated for range $\mathcal{R}$ = [$-\infty$,15) is set as the reference count. For $\mathcal{R}$ = [$-\infty$,8), count($\mathcal{R}$)$_{D}$ generates a value of 0 which is not equal to the current reference count = 2 and for $\mathcal{R}$ = [$-\infty$,8+1), count($\mathcal{R}$)$_{D}$ outputs 2 which is equal to the reference count. This binary search result tell us that V=8 is an element in the database and it is repeats in the database 2-0=2 times. Next, the value  generated for range $\mathcal{R}$ = [$-\infty$,8) is set as the reference count and since the current reference count = 0, the while loop in line 6 of algorithm 10 does not run again. Through the binary search mechanism, algorithm 10 allows us to reconstruct the entire database.
% \end{example}

% \begin{example}
% To illustrate how the reconstruction will function, let's consider a Database, D = [8,8,15] and assume K=1. Initially calling algorithm 9 by setting u and v to be very large, let's call this range $\mathcal{R}$ = [$-\infty$,$\infty$), will return the count of the entire database, D. In our example, count($\mathcal{R}$)$_{D}$ = 3. This size of the the database will be set as the first current reference count.  Now, in algorithm 9, a binary search will be  performed over possible values of v such that for range $\mathcal{R}$ = [$-\infty$,v), count($\mathcal{R}$)$_{D}$ will generate a value of X which is not equal to the current reference count = 3 and range $\mathcal{R}$ = [$-\infty$,v + smallest increment) (smallest increment is 1 for data-sets that only contains integer value elements) generates count($\mathcal{R}$)$_{D}$ = current reference count. In database, D, for $\mathcal{R}$ = [$-\infty$,15), count($\mathcal{R}$)$_{D}$ generates a value of 2 which is not equal to 3 and for  $\mathcal{R}$ = [$-\infty$,15+1), count($\mathcal{R}$)$_{D}$ generates an output equal to 3. This binary search results tell us that V=15 is an element in the database and it repeats in the database 3-2=1 times. Next, the value  generated for range $\mathcal{R}$ = [$-\infty$,15) is set as the reference count. For $\mathcal{R}$ = [$-\infty$,8), count($\mathcal{R}$)$_{D}$ generates a value of 0 which is not equal to the current reference count = 2 and for $\mathcal{R}$ = [$-\infty$,8+1), count($\mathcal{R}$)$_{D}$ outputs 2 which is equal to the reference count. This binary search result tell us that V=8 is an element in the database and it is repeats in the database 2-0=2 times. Next, the value  generated for range $\mathcal{R}$ = [$-\infty$,8) is set as the reference count and since the current reference count = 0, the while loop in line 6 of algorithm 10 does not run again. Through the binary search mechanism, algorithm 10 allows us to reconstruct the entire database.
% \end{example}

% \begin{lem}
% \label{lem:groupKBoundary}
% Given a function $f_{b,u,v}$ as defined in Equation \ref{eqn:fnv}, and group size, K $>$ size(Database) $<$ 2 K, if the count of an element, Count(element) + K $\geq$ database.size() and Count(element) - K $\leq$ 0, our reconstruction mechanism would be able to identify the element being in the database but only an estimate of the upper bound and lower bound of the true count of the element can be inferred from the reconstruction algorithm.
% \end{lem}

% \begin{proof}
% Let $a_1 \le a_2 \le \cdots \le a_k \le a_{k+1} \le \cdots \le a_{k+m-1} \le a_n$ be the elements of database $D$ in non-decreasing order where $a_k$ is the first element of D within the range $\left[u, v\right)$, and $a_{k+m-1}$ is the final element of D in the range (i.e. there are $m$ elements in the range), and $m \ge 2$. We will also define $\mathcal{R}$ to be the range: $\mathcal{R}$ = $\left[u, v\right)$.

% We note that the value of a count function queried on neighboring database D' varies by a maximum of K in either the positive or negative direction from the value of a count function with the same parameters queried on D. Specifically, it has a range of $max(0, m - K)$ to $min(size(D), m + K)$ inclusive. This is because a neighboring database can differ by only K records under group differential privacy.

% If $b < m - K$, then the lowest possible value for $count(\mathcal{R})_{D'}$ is equal to $m - K$, in which case $f_{b,u,v}$ would evaluate to 1 on such a D' because we have $b < m - K$ by definition of b. Since we can clearly see that $f_{b,u,v}$ would evaluate to 1 on D, the K-local sensitivity of $f_{b,u,v}$ in this case must be 0.

% Similarly, if $b \ge m + K$, then the greatest possible value for $count(\mathcal{R})_{D'}$ is equal to $m + K$, in which case $f_{b,u,v}$ would evaluate to 0 on such a D' because we have $b \ge m + K$ by definition of b, which implies that the statement $m > b$ would be false. Since we can clearly see that $f_{b,u,v}$ would evaluate to 0 on D (since b is defined as greater than or equal to $m+K$), we can see that the K-local sensitivity of $f_{b,u,v}$ in this case must be 0.

% However, if b is in the range $m-K \le b < m+K$, then we see that a neighboring database could be constructed with a different evaluation of $f_{b,u,v}$. We note that $f_{b,u,v}$ evaluates to 1 on D when $m - K \le b < m$. However, we can construct a neighboring database D' with up to K fewer entries in $\mathcal{R}$. On this database, the inequality $b < count(\mathcal{R})_{D'} - 1$ would be false, and $f_{b,u,v}$ would evaluate to 0. Thus, the function would have a K-local sensitivity of 1. 

% Similarly, if we have $m \le b < m + K$, then $f_{b,u,v}$ would evaluate to 0 on D. However, we could construct a neighboring database D' with up to K more entries in $\mathcal{R}$. On this database, we would have $b < count(\mathcal{R})_{D'} + 1$, and $f_{b,u,v}$ would evaluate to 1. Thus, the function would have a K-local sensitivity of 1.
% \end{proof}
